GenH2R: Learning Generalizable Human-to-Robot Handover via Scalable Simulation, Demonstration, and Imitation

This paper presents GenH2R, a framework for learning generalizable vision-based human-to-robot (H2R) handover skills. The goal is to equip robots with the ability to reliably receive objects with unseen geometry handed over by humans in various complex trajectories. We acquire such generalizability by learning H2R handover at scale with a comprehensive solution including procedural simulation assets creation, automated demonstration generation, and effective imitation learning. We leverage large-scale 3D model repositories, dexterous grasp generation methods, and curve-based 3D animation to create an H2R handover simulation environment named \simabbns, surpassing the number of scenes in existing simulators by three orders of magnitude. We further introduce a distillation-friendly demonstration generation method that automatically generates a million high-quality demonstrations suitable for learning. Finally, we present a 4D imitation learning method augmented by a future forecasting objective to distill demonstrations into a visuo-motor handover policy. Experimental evaluations in both simulators and the real world demonstrate significant improvements (at least +10\% success rate) over baselines in all cases. The project page is https://GenH2R.github.io/.

==> tables/different_time_wait.tex <==
% % \begin{table*}[t]
% %  % \vspace{-2mm}
% %  \centering
% %  \small
% %  % \setlength{\tabcolsep}{6pt}
% %  \begin{tabular}{l|l|cc|cc|cc|cc}

% %   \hline
% %     & & \multicolumn{2}{c|}{S0~(Sequential)} & \multicolumn{2}{c|}{S0~ (Simult.)}  & \multicolumn{2}{c|}{T0} & \multicolumn{2}{c}{T1}\\
% %   & & success(\%) & time(s) & success(\%) & time(s) & success(\%) & time(s) & success(\%) & time(s)\\
% %   \hline
% %   % \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Trained on S0}}} \\
% %   % \parbox[t]{6mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Trained on S0}}} \\
% %    OMG Planner~\cite{wang:rss2020} $\dagger$    &  &  62.50 &          - &  -  & & & & &\\
% %    % Vision Planner~\cite{wang:rss2020} $\dagger$        & &          &    & & & & &   \\
% %      \cline{3-10}
% %    % \hline

   
% % % \cline{2-10}
% %    GA-DDPG~\cite{wang2022goal} &  & 50.00 &  7.34        &   36.81 & 4.58 & 23.59 & 7.31 & &        \\
% %   % & \gc GA-DDPG~\cite{wang:corl2021b} finetuned  & \gc 57.18         & \gc  \textbf{6.324}        & \gc \textbf{0.086} & \gc \textbf{6.411}      & \gc ~6.48 &  \gc 27.08          &  \gc ~9.26  & \gc 42.82      \\
 
% %    Handover-sim2real~\cite{christen2023learning} &  & 75.23 &    7.71      &  68.75  & 6.19& 31.34 & 6.21& &    \\

% %    \cline{2-10}

   
% %    Ours~(Replan 1)  &  & &          &    & & & & &      \\
% %    Ours~(Know Dest.) &   & &          &    & & & & &    \\
% %    Ours~(Landmark)  &  & &          &    & & & & &         \\
% % %   & \gc Ours + grasp pred. & \gc 71.07 & \gc 5.43 & \gc tbd & \gc tbd  & \gc ~6.00 & \gc 16.20 & \gc ~6.73 \\ 
% % %   Ours (hand avg + pred)  w/o hold & 43.73 & tbd & tbd & tbd  & 16.3 & ~21.5 & ~18.40 \\ 
% % % \hline
% % %   & \gc Ours + grasp pred & \gc 70.37 & \gc 4.860 & \gc tbd & \gc tbd  & \gc 7.64 & \gc ~14.71 & \gc ~6.95 \\ 
  
% % \bottomrule
  
% %  \end{tabular}
% %  \vspace{-1mm}
% %  \caption{\textbf{HandoverSim Benchmark Evaluation trained on S0.} We compare our method against various baselines from the test set of HandoverSim benchmark\cite{chao2022handoversim} (\textit{S0~Sequential} and \textit{S0~Simultaneous}) and our proposed benchmark (\textit{T0} and \textit{T1}). We use the best-pretrained models from the repositories of \textbf{GA-DDPG}~\cite{wang2022goal} and \textbf{Handover-Sim2real}~\cite{christen2023learning}. And our models are trained in the train set of S0. 
% % The results for our method are averaged across 3 random seeds. $\dagger$: This method \cite{wang:rss2020} is evaluated with ground-truth states.
% % % and thus are not directly comparable with ours.
% % }
% %  \vspace{-1em}
% %  \label{tab:quantitative}
% % \end{table*}


% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[t]
% \centering
% \small
% \begin{tabular}{cc|ccc|ccc|ccc|ccc}
% \hline
% \multicolumn{2}{c|}{\multirow{2}{*}{}}                                    & \multicolumn{3}{c|}{ -s0(Sequential)}         & \multicolumn{3}{c|}{s0 (Simultaneous)}            & \multicolumn{3}{c|}{t0}                      & \multicolumn{3}{c}{t1}                      \\
% \multicolumn{2}{c|}{}                                                     & Suc.          & T   &  AS        & Suc.          & T  &  AS            & Suc.         & T   &  AS  & Suc.          & T  &  AS          \\ \hline
%  & OMG Planner~\cite{wang:rss2020} $\dagger$ & 62.50 &  8.31  &  0.23&   &  &  &    &    &         &       &      &                       \\ \cline{1-14} 

% \multicolumn{1}{c|}{\multirow{6}{*}{(HandoverSim)}} & GA-DDPG~\cite{wang2022goal}  & 50.00 &  \textbf{7.14} & 0.23 & 36.81 & \textbf{4.66} & 0.24 & 23.59 & 7.31 & 0.10 & 46.7 & 5.50 & 0.27\\

% \multicolumn{1}{c|}{\multirow{2}{*}{train on s0}}   & Handover-Sim2real~\cite{christen2023learning}   & 75.23 &    7.74  &  0.30  &  68.75  & 6.23 & 0.36 & 30.34 & 6.21& 0.16 & 52.4 & 7.09 & 0.24\\
% \cline{2-14}

% \multicolumn{1}{c|}{} &  Destination Planning   &  74.31 &  7.98 & 0.29 & 76.16 & 5.89 & 0.42 & 25.68 & 5.34 & 0.15 & & & \\

% \multicolumn{1}{c|}{} & Dense Planning  & 74.77 & 8.14 & 0.28  & 75.45 & 6.06 &  0.40 &   27.30 & 5.49 & 0.16 & 52.3 & 7.44 & 0.22 \\


% \multicolumn{1}{c|}{} & Landmark Planning  & 77.78 & 8.15 & 0.29 & 79.17 & 6.06 & 0.42 & 29.63 & 5.22 & 0.18 & 54.2 & 7.41 & 0.23\\  
% \hline
% \hline
% % \cline{2-10}

% % \multicolumn{1}{c|}{\multirow{6}{*}{train on t0}} & OMG Planner~\cite{wang:rss2020} $\dagger$ &  &    &     &        &             &       &      &                       \\ \cline{2-10} 

% % \multicolumn{1}{c|}{\multirow{6}{*}{train on t0}} & GA-DDPG~\cite{wang2022goal}   &  &   &  &  &  &  & &  \\

% % \multicolumn{1}{c|}{}  & Handover-Sim2real~\cite{christen2023learning}    &  &   &  &  &  &  & & \\
% \cline{2-14}

% \multicolumn{1}{c|}{\multirow{2.5}{*}{train on t0}} & Destination Planning   & 0.93 &  11.76 & 0.00 & 6.48 & 11.22 & 0.01 & 5.96 & 7.57 & 0.03 & 1.60 & 11.38 & 0.00\\
% % Test_t450_t450_bc_omg_know_dest_use_hand_flow0_pred0_new_no_accum
% % Test_s0_t450_bc_omg_know_dest_use_hand_flow0_pred0_new_no_accum

% \multicolumn{1}{c|}{\multirow{2.5}{*}{(\simabbns)}} & Dense Planning  & 80.79 & 8.59 & 0.27 & \textbf{86.81} & 6.41 & 0.44 & 39.04 & 5.81 & 0.22 
% & 64.2 &  7.24 & 0.284\\
% % Test_t450_t450_bc_omg_replan1_smooth0.08_use_hand_flow0_pred0_no_accum
% % Test_s0_t450_bc_omg_replan1_smooth0.08_use_hand_flow0_pred0_no_accum


% \multicolumn{1}{c|}{} & Landmark Planning & \textbf{87.27} & 7.66 & \textbf{0.36} & 84.03  & 5.57 & \textbf{0.48} & 40.43 &  4.85 & 0.25 & 62.4 &  6.20 & 0.33\\  
% % Test_t450_t450_bc_omg_replan5_landmark_smooth0.08_use_hand_flow3_pred3_wd0.0001_pred0.5_no_accum
% % Test_s0_t450_bc_omg_replan5_landmark_smooth0.08_use_hand_flow3_pred3_wd0.0001_pred0.5_no_accum

% \hline
% \end{tabular}
% \vspace{-1mm}
%  \caption{\textbf{HandoverSim Benchmark Evaluation trained on S0.} We compare our method against various baselines from the test set of HandoverSim benchmark\cite{chao2022handoversim} (\textit{S0~Sequential} and \textit{S0~Simultaneous}) and our proposed benchmark (\textit{T0} and \textit{T1}). We use the best-pretrained models from the repositories of \textbf{GA-DDPG}~\cite{wang2022goal} and \textbf{Handover-Sim2real}~\cite{christen2023learning}. And our models are trained in the train set of S0. 
% The results for our method are averaged across 3 random seeds. $\dagger$: This method \cite{wang:rss2020} is evaluated with ground-truth states.
% % and thus are not directly comparable with ours.
% }
%  \vspace{-1em}
%  \label{tab:main_exp}
% \end{table*}





% \begin{table*}[t]
%  % \vspace{-2mm}
%  \centering
%  \small
%  % \setlength{\tabcolsep}{6pt}
%  \begin{tabular}{l|l|cc|cc|cc|cc}

%   \hline
%     & & \multicolumn{2}{c|}{S0~(Sequential)} & \multicolumn{2}{c|}{S0~ (Simult.)}  & \multicolumn{2}{c|}{T0} & \multicolumn{2}{c}{T1}\\
%   & & success(\%) & time(s) & success(\%) & time(s) & success(\%) & time(s) & success(\%) & time(s)\\
%   \hline
%   % \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Trained on S0}}} \\
%   % \parbox[t]{6mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Trained on S0}}} \\
%    OMG Planner~\cite{wang:rss2020} $\dagger$    &  &  62.50 &          - &  -  & & & & &\\
%    % Vision Planner~\cite{wang:rss2020} $\dagger$        & &          &    & & & & &   \\
%      \cline{3-10}
%    % \hline

   
% % \cline{2-10}
%    GA-DDPG~\cite{wang2022goal} &  & 50.00 &  7.34        &   36.81 & 4.58 & 23.59 & 7.31 & &        \\
%   % & \gc GA-DDPG~\cite{wang:corl2021b} finetuned  & \gc 57.18         & \gc  \textbf{6.324}        & \gc \textbf{0.086} & \gc \textbf{6.411}      & \gc ~6.48 &  \gc 27.08          &  \gc ~9.26  & \gc 42.82      \\
 
%    Handover-sim2real~\cite{christen2023learning} &  & 75.23 &    7.71      &  68.75  & 6.19& 31.34 & 6.21& &    \\

%    \cline{2-10}

   
%    Ours~(Replan 1)  &  & &          &    & & & & &      \\
%    Ours~(Know Dest.) &   & &          &    & & & & &    \\
%    Ours~(Landmark)  &  & &          &    & & & & &         \\
% %   & \gc Ours + grasp pred. & \gc 71.07 & \gc 5.43 & \gc tbd & \gc tbd  & \gc ~6.00 & \gc 16.20 & \gc ~6.73 \\ 
% %   Ours (hand avg + pred)  w/o hold & 43.73 & tbd & tbd & tbd  & 16.3 & ~21.5 & ~18.40 \\ 
% % \hline
% %   & \gc Ours + grasp pred & \gc 70.37 & \gc 4.860 & \gc tbd & \gc tbd  & \gc 7.64 & \gc ~14.71 & \gc ~6.95 \\ 
  
% \bottomrule
  
%  \end{tabular}
%  \vspace{-1mm}
%  \caption{\textbf{HandoverSim Benchmark Evaluation trained on S0.} We compare our method against various baselines from the test set of HandoverSim benchmark\cite{chao2022handoversim} (\textit{S0~Sequential} and \textit{S0~Simultaneous}) and our proposed benchmark (\textit{T0} and \textit{T1}). We use the best-pretrained models from the repositories of \textbf{GA-DDPG}~\cite{wang2022goal} and \textbf{Handover-Sim2real}~\cite{christen2023learning}. And our models are trained in the train set of S0. 
% The results for our method are averaged across 3 random seeds. $\dagger$: This method \cite{wang:rss2020} is evaluated with ground-truth states.
% % and thus are not directly comparable with ours.
% }
%  \vspace{-1em}
%  \label{tab:quantitative}
% \end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
\small
\begin{tabular}{c|ccc|ccc|ccc|ccc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{}}                                    & \multicolumn{3}{c|}{s0 (Sequential)}         & \multicolumn{3}{c|}{s0 (Simultaneous)}            & \multicolumn{3}{c|}{t0}                      & \multicolumn{3}{c}{t1}                      \\
\multicolumn{1}{c|}{}                                                     & S          & T   &  AS        & S          & T  &  AS            & S         & T   &  AS  & S          & T  &  AS          \\ \hline
% \hline
% \cline{2-10}

% \multicolumn{1}{c|}{\multirow{6}{*}{train on t0}} & OMG Planner~\cite{wang:rss2020} $\dagger$ &  &    &     &        &             &       &      &                       \\ \cline{2-10} 
 Handover-Sim2real~\cite{christen2023learning} (WAIT = 1.5s)    &  65.97 &  7.18  & 29.5 & 62.50 & 6.04 & 33.5 & 33.71 & 5.91 & 18.4 & 47.10 & 6.35 & 24.1\\
 
Handover-Sim2real~\cite{christen2023learning} (WAIT = 0s)   &  65.97 &  7.18  & 29.5 & 34.72 &  5.27 & 20.6 & 32.46 & 4.65 & 21.0 & 36.90 & 5.85 & 20.3\\
 
\hline
% Test_t450_t450_bc_omg_replan5_landmark_smooth0.08_use_hand_flow3_pred3_wd0.0001_pred0.5_no_accum
% Test_s0_t450_bc_omg_replan5_landmark_smooth0.08_use_hand_flow3_pred3_wd0.0001_pred0.5_no_accum

\end{tabular}
\vspace{-1mm}
 \caption{\textbf{Different TIME\_WAIT parameters for Handover-Sim2real. }
When comparing different values for TIME\_WAIT, we observe that setting TIME\_WAIT to 0s results in a decrease in performance for the simultaneous settings.
% and thus are not directly comparable with ours.
}
 \vspace{-1em}
 \label{tab:wait_time}
\end{table*}

==> tables/grasp_generating.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{3mm}
\small
\begin{tabular}{cccc}
\hline
\textbf{Methods}              & Scale & Real/Synthetic &  Shapenet(Y/N)\\ \hline
DexYCB            &     999       &   Real    &  N\\ 
HOI4D       &  4,000     &     Real        &      N\\
OBMAN   &    21,000      &   Synthetic &    Y\\ 
\textbf{DexGraspNet} & 1,000,000 & Synthetic & Y \\

\hline


\end{tabular}
\vspace{-1mm}
 \caption{\textbf{Human-object grasps by different methods.} ``Gen(Y/N)'' means whether the objects in the corresponding dataset belong to ShapeNet~\cite{chang2015shapenet} dataset. Only objects in ShapeNet are suitable for physics simulation~\cite{eppner2021acronym} to generate candidate grasps for the robotic arm.
% and thus are not directly comparable with ours.
}
 \vspace{-1em}
 \label{tab:grasp}
\end{table}

==> tables/poster_table.tex <==
% % \begin{table*}[t]
% %  % \vspace{-2mm}
% %  \centering
% %  \small
% %  % \setlength{\tabcolsep}{6pt}
% %  \begin{tabular}{l|l|cc|cc|cc|cc}

% %   \hline
% %     & & \multicolumn{2}{c|}{S0~(Sequential)} & \multicolumn{2}{c|}{S0~ (Simult.)}  & \multicolumn{2}{c|}{T0} & \multicolumn{2}{c}{T1}\\
% %   & & success(\%) & time(s) & success(\%) & time(s) & success(\%) & time(s) & success(\%) & time(s)\\
% %   \hline
% %   % \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Trained on S0}}} \\
% %   % \parbox[t]{6mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Trained on S0}}} \\
% %    OMG Planner~\cite{wang:rss2020} $\dagger$    &  &  62.50 &          - &  -  & & & & &\\
% %    % Vision Planner~\cite{wang:rss2020} $\dagger$        & &          &    & & & & &   \\
% %      \cline{3-10}
% %    % \hline

   
% % % \cline{2-10}
% %    GA-DDPG~\cite{wang2022goal} &  & 50.00 &  7.34        &   36.81 & 4.58 & 23.59 & 7.31 & &        \\
% %   % & \gc GA-DDPG~\cite{wang:corl2021b} finetuned  & \gc 57.18         & \gc  \textbf{6.324}        & \gc \textbf{0.086} & \gc \textbf{6.411}      & \gc ~6.48 &  \gc 27.08          &  \gc ~9.26  & \gc 42.82      \\
 
% %    Handover-sim2real~\cite{christen2023learning} &  & 75.23 &    7.71      &  68.75  & 6.19& 31.34 & 6.21& &    \\

% %    \cline{2-10}

   
% %    Ours~(Replan 1)  &  & &          &    & & & & &      \\
% %    Ours~(Know Dest.) &   & &          &    & & & & &    \\
% %    Ours~(Landmark)  &  & &          &    & & & & &         \\
% % %   & \gc Ours + grasp pred. & \gc 71.07 & \gc 5.43 & \gc tbd & \gc tbd  & \gc ~6.00 & \gc 16.20 & \gc ~6.73 \\ 
% % %   Ours (hand avg + pred)  w/o hold & 43.73 & tbd & tbd & tbd  & 16.3 & ~21.5 & ~18.40 \\ 
% % % \hline
% % %   & \gc Ours + grasp pred & \gc 70.37 & \gc 4.860 & \gc tbd & \gc tbd  & \gc 7.64 & \gc ~14.71 & \gc ~6.95 \\ 
  
% % \bottomrule
  
% %  \end{tabular}
% %  \vspace{-1mm}
% %  \caption{\textbf{HandoverSim Benchmark Evaluation trained on S0.} We compare our method against various baselines from the test set of HandoverSim benchmark\cite{chao2022handoversim} (\textit{S0~Sequential} and \textit{S0~Simultaneous}) and our proposed benchmark (\textit{T0} and \textit{T1}). We use the best-pretrained models from the repositories of \textbf{GA-DDPG}~\cite{wang2022goal} and \textbf{Handover-Sim2real}~\cite{christen2023learning}. And our models are trained in the train set of S0. 
% % The results for our method are averaged across 3 random seeds. $\dagger$: This method \cite{wang:rss2020} is evaluated with ground-truth states.
% % % and thus are not directly comparable with ours.
% % }
% %  \vspace{-1em}
% %  \label{tab:quantitative}
% % \end{table*}


% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[t]
% \centering
% \small
% \begin{tabular}{cc|ccc|ccc|ccc|ccc}
% \hline
% \multicolumn{2}{c|}{\multirow{2}{*}{}}                                    & \multicolumn{3}{c|}{ -s0(Sequential)}         & \multicolumn{3}{c|}{s0 (Simultaneous)}            & \multicolumn{3}{c|}{t0}                      & \multicolumn{3}{c}{t1}                      \\
% \multicolumn{2}{c|}{}                                                     & Suc.          & T   &  AS        & Suc.          & T  &  AS            & Suc.         & T   &  AS  & Suc.          & T  &  AS          \\ \hline
%  & OMG Planner~\cite{wang:rss2020} $\dagger$ & 62.50 &  8.31  &  0.23&   &  &  &    &    &         &       &      &                       \\ \cline{1-14} 

% \multicolumn{1}{c|}{\multirow{6}{*}{(HandoverSim)}} & GA-DDPG~\cite{wang2022goal}  & 50.00 &  \textbf{7.14} & 0.23 & 36.81 & \textbf{4.66} & 0.24 & 23.59 & 7.31 & 0.10 & 46.7 & 5.50 & 0.27\\

% \multicolumn{1}{c|}{\multirow{2}{*}{train on s0}}   & Handover-Sim2real~\cite{christen2023learning}   & 75.23 &    7.74  &  0.30  &  68.75  & 6.23 & 0.36 & 30.34 & 6.21& 0.16 & 52.4 & 7.09 & 0.24\\
% \cline{2-14}

% \multicolumn{1}{c|}{} &  Destination Planning   &  74.31 &  7.98 & 0.29 & 76.16 & 5.89 & 0.42 & 25.68 & 5.34 & 0.15 & & & \\

% \multicolumn{1}{c|}{} & Dense Planning  & 74.77 & 8.14 & 0.28  & 75.45 & 6.06 &  0.40 &   27.30 & 5.49 & 0.16 & 52.3 & 7.44 & 0.22 \\


% \multicolumn{1}{c|}{} & Landmark Planning  & 77.78 & 8.15 & 0.29 & 79.17 & 6.06 & 0.42 & 29.63 & 5.22 & 0.18 & 54.2 & 7.41 & 0.23\\  
% \hline
% \hline
% % \cline{2-10}

% % \multicolumn{1}{c|}{\multirow{6}{*}{train on t0}} & OMG Planner~\cite{wang:rss2020} $\dagger$ &  &    &     &        &             &       &      &                       \\ \cline{2-10} 

% % \multicolumn{1}{c|}{\multirow{6}{*}{train on t0}} & GA-DDPG~\cite{wang2022goal}   &  &   &  &  &  &  & &  \\

% % \multicolumn{1}{c|}{}  & Handover-Sim2real~\cite{christen2023learning}    &  &   &  &  &  &  & & \\
% \cline{2-14}

% \multicolumn{1}{c|}{\multirow{2.5}{*}{train on t0}} & Destination Planning   & 0.93 &  11.76 & 0.00 & 6.48 & 11.22 & 0.01 & 5.96 & 7.57 & 0.03 & 1.60 & 11.38 & 0.00\\
% % Test_t450_t450_bc_omg_know_dest_use_hand_flow0_pred0_new_no_accum
% % Test_s0_t450_bc_omg_know_dest_use_hand_flow0_pred0_new_no_accum

% \multicolumn{1}{c|}{\multirow{2.5}{*}{(\simabbns)}} & Dense Planning  & 80.79 & 8.59 & 0.27 & \textbf{86.81} & 6.41 & 0.44 & 39.04 & 5.81 & 0.22 
% & 64.2 &  7.24 & 0.284\\
% % Test_t450_t450_bc_omg_replan1_smooth0.08_use_hand_flow0_pred0_no_accum
% % Test_s0_t450_bc_omg_replan1_smooth0.08_use_hand_flow0_pred0_no_accum


% \multicolumn{1}{c|}{} & Landmark Planning & \textbf{87.27} & 7.66 & \textbf{0.36} & 84.03  & 5.57 & \textbf{0.48} & 40.43 &  4.85 & 0.25 & 62.4 &  6.20 & 0.33\\  
% % Test_t450_t450_bc_omg_replan5_landmark_smooth0.08_use_hand_flow3_pred3_wd0.0001_pred0.5_no_accum
% % Test_s0_t450_bc_omg_replan5_landmark_smooth0.08_use_hand_flow3_pred3_wd0.0001_pred0.5_no_accum

% \hline
% \end{tabular}
% \vspace{-1mm}
%  \caption{\textbf{HandoverSim Benchmark Evaluation trained on S0.} We compare our method against various baselines from the test set of HandoverSim benchmark\cite{chao2022handoversim} (\textit{S0~Sequential} and \textit{S0~Simultaneous}) and our proposed benchmark (\textit{T0} and \textit{T1}). We use the best-pretrained models from the repositories of \textbf{GA-DDPG}~\cite{wang2022goal} and \textbf{Handover-Sim2real}~\cite{christen2023learning}. And our models are trained in the train set of S0. 
% The results for our method are averaged across 3 random seeds. $\dagger$: This method \cite{wang:rss2020} is evaluated with ground-truth states.
% % and thus are not directly comparable with ours.
% }
%  \vspace{-1em}
%  \label{tab:main_exp}
% \end{table*}





% \begin{table*}[t]
%  % \vspace{-2mm}
%  \centering
%  \small
%  % \setlength{\tabcolsep}{6pt}
%  \begin{tabular}{l|l|cc|cc|cc|cc}

%   \hline
%     & & \multicolumn{2}{c|}{S0~(Sequential)} & \multicolumn{2}{c|}{S0~ (Simult.)}  & \multicolumn{2}{c|}{T0} & \multicolumn{2}{c}{T1}\\
%   & & success(\%) & time(s) & success(\%) & time(s) & success(\%) & time(s) & success(\%) & time(s)\\
%   \hline
%   % \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Trained on S0}}} \\
%   % \parbox[t]{6mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Trained on S0}}} \\
%    OMG Planner~\cite{wang:rss2020} $\dagger$    &  &  62.50 &          - &  -  & & & & &\\
%    % Vision Planner~\cite{wang:rss2020} $\dagger$        & &          &    & & & & &   \\
%      \cline{3-10}
%    % \hline

   
% % \cline{2-10}
%    GA-DDPG~\cite{wang2022goal} &  & 50.00 &  7.34        &   36.81 & 4.58 & 23.59 & 7.31 & &        \\
%   % & \gc GA-DDPG~\cite{wang:corl2021b} finetuned  & \gc 57.18         & \gc  \textbf{6.324}        & \gc \textbf{0.086} & \gc \textbf{6.411}      & \gc ~6.48 &  \gc 27.08          &  \gc ~9.26  & \gc 42.82      \\
 
%    Handover-sim2real~\cite{christen2023learning} &  & 75.23 &    7.71      &  68.75  & 6.19& 31.34 & 6.21& &    \\

%    \cline{2-10}

   
%    Ours~(Replan 1)  &  & &          &    & & & & &      \\
%    Ours~(Know Dest.) &   & &          &    & & & & &    \\
%    Ours~(Landmark)  &  & &          &    & & & & &         \\
% %   & \gc Ours + grasp pred. & \gc 71.07 & \gc 5.43 & \gc tbd & \gc tbd  & \gc ~6.00 & \gc 16.20 & \gc ~6.73 \\ 
% %   Ours (hand avg + pred)  w/o hold & 43.73 & tbd & tbd & tbd  & 16.3 & ~21.5 & ~18.40 \\ 
% % \hline
% %   & \gc Ours + grasp pred & \gc 70.37 & \gc 4.860 & \gc tbd & \gc tbd  & \gc 7.64 & \gc ~14.71 & \gc ~6.95 \\ 
  
% \bottomrule
  
%  \end{tabular}
%  \vspace{-1mm}
%  \caption{\textbf{HandoverSim Benchmark Evaluation trained on S0.} We compare our method against various baselines from the test set of HandoverSim benchmark\cite{chao2022handoversim} (\textit{S0~Sequential} and \textit{S0~Simultaneous}) and our proposed benchmark (\textit{T0} and \textit{T1}). We use the best-pretrained models from the repositories of \textbf{GA-DDPG}~\cite{wang2022goal} and \textbf{Handover-Sim2real}~\cite{christen2023learning}. And our models are trained in the train set of S0. 
% The results for our method are averaged across 3 random seeds. $\dagger$: This method \cite{wang:rss2020} is evaluated with ground-truth states.
% % and thus are not directly comparable with ours.
% }
%  \vspace{-1em}
%  \label{tab:quantitative}
% \end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
\small
\begin{tabular}{c|ccc|ccc|ccc|ccc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{}}                                    & \multicolumn{3}{c|}{s0 (Sequential)}         & \multicolumn{3}{c|}{s0 (Simultaneous)}            & \multicolumn{3}{c|}{t0}                      & \multicolumn{3}{c}{t1}                      \\
\multicolumn{1}{c|}{}                                                     & S         &  T    &  AS        & S    & T       &  AS            & S    & T        &  AS  & S      & T     &  AS          \\ \hline
% HandoverSim

% \cline{2-10}

% \multicolumn{1}{c|}{\multirow{6}{*}{train on t0}} & OMG Planner~\cite{wang:rss2020} $\dagger$ &  &    &     &        &             &       &      &                       \\ \cline{2-10} 


\textcolor{black}{Handover-Sim2real}    &  65.97   & 7.18 & 29.5 & 62.50  & 6.04 & 33.5 & 33.71  & 5.91 & 18.4 & 47.10  & 6.35 & 24.1\\


% Test_t450_t450_bc_omg_know_dest_use_hand_flow0_pred0_new_no_accum
% Test_s0_t450_bc_omg_know_dest_use_hand_flow0_pred0_new_no_accum

%simabbns
% Test_t450_t450_bc_omg_replan1_smooth0.08_use_hand_flow0_pred0_no_accum
% Test_s0_t450_bc_omg_replan1_smooth0.08_use_hand_flow0_pred0_no_accum


 Ours & \textbf{86.57}  & 8.81 &  28.0 & \textbf{85.65}   &6.58 & \textbf{42.8} & \textbf{41.43}  & 6.01 &\textbf{22.3} &\textbf{68.33}  & 7.70 & \textbf{27.9}\\  
% Test_t450_t450_bc_omg_replan5_landmark_smooth0.08_use_hand_flow3_pred3_wd0.0001_pred0.5_no_accum
% Test_s0_t450_bc_omg_replan5_landmark_smooth0.08_use_hand_flow3_pred3_wd0.0001_pred0.5_no_accum

\hline
\end{tabular}
\vspace{-1mm}
 \caption{\textbf{Evaluating on different benchmarks. } We compare our method against baselines from the test set of HandoverSim benchmark\cite{chao2022handoversim} (``s0 (sequential)'' and ``s0 (simultaneous)'') and our \simabbns~benchmark (``t0'' and ``t1''). We use the best-pretrained models from the repositories of GA-DDPG~\cite{wang2022goal} and Handover-Sim2real~\cite{christen2023learning} for evaluation. The results for our method are averaged across 3 random seeds. Note that S means success rate(\%). T means time(s). AS means average success(\%) as defined in Equation 2 in the manuscript. $\dagger$: This method \cite{wang:rss2020} is evaluated with ground-truth states and cannot handle dynamic handover like ``s0 (Simultaneous)'', ``t0'' and ``t1''. The methods denoted in \textcolor{blue}{blue} are newly added in the supplementary material and will be included in the manuscript in subsequent revisions.
% and thus are not directly comparable with ours.
}
 \vspace{-1em}
 \label{tab:main_exp_complete}
\end{table*}




\begin{table*}[t]
\centering
\small
\begin{tabular}{c|ccc|ccc|}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{}}                                    & \multicolumn{3}{c|}{s0 (Sequential)}         & \multicolumn{3}{c|}{s0 (Simultaneous)}                          \\
\multicolumn{1}{c|}{}                                                     & S         &  T    &  AS        & S    & T       &  AS              \\ \hline
% HandoverSim

% \cline{2-10}

% \multicolumn{1}{c|}{\multirow{6}{*}{train on t0}} & OMG Planner~\cite{wang:rss2020} $\dagger$ &  &    &     &        &             &       &      &                       \\ \cline{2-10} 


\textcolor{black}{Handover-Sim2real}    &  65.97   & 7.18 & 29.5 & 62.50  & 6.04 & 33.5 \\


% Test_t450_t450_bc_omg_know_dest_use_hand_flow0_pred0_new_no_accum
% Test_s0_t450_bc_omg_know_dest_use_hand_flow0_pred0_new_no_accum

%simabbns
% Test_t450_t450_bc_omg_replan1_smooth0.08_use_hand_flow0_pred0_no_accum
% Test_s0_t450_bc_omg_replan1_smooth0.08_use_hand_flow0_pred0_no_accum


 Ours & \textbf{86.57}  & 8.81 &  28.0 & \textbf{85.65}   &6.58 & \textbf{42.8} \\  
% Test_t450_t450_bc_omg_replan5_landmark_smooth0.08_use_hand_flow3_pred3_wd0.0001_pred0.5_no_accum
% Test_s0_t450_bc_omg_replan5_landmark_smooth0.08_use_hand_flow3_pred3_wd0.0001_pred0.5_no_accum

\hline
\end{tabular}
\vspace{-1mm}
 \caption{\textbf{Evaluating on different benchmarks. } We compare our method against baselines from the test set of HandoverSim benchmark\cite{chao2022handoversim} (``s0 (sequential)'' and ``s0 (simultaneous)'') and our \simabbns~benchmark (``t0'' and ``t1''). We use the best-pretrained models from the repositories of GA-DDPG~\cite{wang2022goal} and Handover-Sim2real~\cite{christen2023learning} for evaluation. The results for our method are averaged across 3 random seeds. Note that S means success rate(\%). T means time(s). AS means average success(\%) as defined in Equation 2 in the manuscript. $\dagger$: This method \cite{wang:rss2020} is evaluated with ground-truth states and cannot handle dynamic handover like ``s0 (Simultaneous)'', ``t0'' and ``t1''. The methods denoted in \textcolor{blue}{blue} are newly added in the supplementary material and will be included in the manuscript in subsequent revisions.
% and thus are not directly comparable with ours.
}
 \vspace{-1em}
 \label{tab:main_exp_complete1}
\end{table*}




\begin{table*}[t]
\centering
\small
\begin{tabular}{c|ccc|ccc|}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{}}                                    &  \multicolumn{3}{c|}{t0}                      & \multicolumn{3}{c}{t1}                      \\
\multicolumn{1}{c|}{}                                                      & S    & T        &  AS  & S      & T     &  AS          \\ \hline
% HandoverSim

% \cline{2-10}

% \multicolumn{1}{c|}{\multirow{6}{*}{train on t0}} & OMG Planner~\cite{wang:rss2020} $\dagger$ &  &    &     &        &             &       &      &                       \\ \cline{2-10} 


\textcolor{black}{Handover-Sim2real}   & 33.71  & 5.91 & 18.4 & 47.10  & 6.35 & 24.1\\


% Test_t450_t450_bc_omg_know_dest_use_hand_flow0_pred0_new_no_accum
% Test_s0_t450_bc_omg_know_dest_use_hand_flow0_pred0_new_no_accum

%simabbns
% Test_t450_t450_bc_omg_replan1_smooth0.08_use_hand_flow0_pred0_no_accum
% Test_s0_t450_bc_omg_replan1_smooth0.08_use_hand_flow0_pred0_no_accum


 Ours & \textbf{41.43}  & 6.01 &\textbf{22.3} &\textbf{68.33}  & 7.70 & \textbf{27.9}\\  
% Test_t450_t450_bc_omg_replan5_landmark_smooth0.08_use_hand_flow3_pred3_wd0.0001_pred0.5_no_accum
% Test_s0_t450_bc_omg_replan5_landmark_smooth0.08_use_hand_flow3_pred3_wd0.0001_pred0.5_no_accum

\hline
\end{tabular}
\vspace{-1mm}
 \caption{\textbf{Evaluating on different benchmarks. } We compare our method against baselines from the test set of HandoverSim benchmark\cite{chao2022handoversim} (``s0 (sequential)'' and ``s0 (simultaneous)'') and our \simabbns~benchmark (``t0'' and ``t1''). We use the best-pretrained models from the repositories of GA-DDPG~\cite{wang2022goal} and Handover-Sim2real~\cite{christen2023learning} for evaluation. The results for our method are averaged across 3 random seeds. Note that S means success rate(\%). T means time(s). AS means average success(\%) as defined in Equation 2 in the manuscript. $\dagger$: This method \cite{wang:rss2020} is evaluated with ground-truth states and cannot handle dynamic handover like ``s0 (Simultaneous)'', ``t0'' and ``t1''. The methods denoted in \textcolor{blue}{blue} are newly added in the supplementary material and will be included in the manuscript in subsequent revisions.
% and thus are not directly comparable with ours.
}
 \vspace{-1em}
 \label{tab:main_exp_complete}
\end{table*}
